Observation of the decay $J/\psi \to e^+ e^- \eta(1405)$ with $\eta(1405) \to \pi^0 f_0(980)$

Using a data sample of $(10087\pm44)\times 10^6$ $J/\psi$ events collected by the BESIII detector in 2009, 2012, 2018 and 2019, the electromagnetic Dalitz process $J/\psi \to e^+ e^- \eta(1405)$ is observed via the decay $\eta(1405) \to \pi^0 f_0(980)$, $f_0(980) \to \pi^+ \pi^-$, with a significance of about $9.6\sigma$. The branching fraction of this decay is measured to be ${\mathcal B}(J/\psi \to e^+ e^- \pi^0 \eta(1405) \to e^+ e^- \pi^0 f_0(980) \to e^+ e^- \pi^0 \pi^+ \pi^-)=(2.02\pm0.24(\rm{stat.})\pm0.09(\rm{syst.}))\times 10^{-7}$. The branching-fraction ratio ${\mathcal B}(J/\psi \to e^+ e^- \eta(1405))$/${\mathcal B}(J/\psi \to \gamma \eta(1405))$ is determined to be $(1.35\pm0.19(\rm{stat.})\pm0.06(\rm{syst.}))\times10^{-2}$. Furthermore, an $e^+e^-$ invariant-mass dependent transition form factor of $J/\psi \to e^+ e^-\eta(1405)$ is presented for the first time. The obtained result provides input for different theoretical models, and is valuable for the improved understanding the intrinsic structure of the $\eta(1405)$ meson.

==> acknowledgement_2023-03-05.tex <==
%% Saved at => 2023-03-05
\textbf{Acknowledgement}

The BESIII Collaboration thanks the staff of BEPCII and the IHEP computing center for their strong support. This work is supported in part by National Key R\&D Program of China under Contracts Nos. 2020YFA0406300, 2020YFA0406400; National Natural Science Foundation of China (NSFC) under Contracts Nos. 11635010, 11735014, 11835012, 11935015, 11935016, 11935018, 11961141012, 12022510, 12025502, 12035009, 12035013, 12061131003, 12192260, 12192261, 12192262, 12192263, 12192264, 12192265, 12221005, 12225509, 12235017; the Chinese Academy of Sciences (CAS) Large-Scale Scientific Facility Program; the CAS Center for Excellence in Particle Physics (CCEPP); CAS Key Research Program of Frontier Sciences under Contracts Nos. QYZDJ-SSW-SLH003, QYZDJ-SSW-SLH040; 100 Talents Program of CAS; The Institute of Nuclear and Particle Physics (INPAC) and Shanghai Key Laboratory for Particle Physics and Cosmology; ERC under Contract No. 758462; European Union's Horizon 2020 research and innovation programme under Marie Sklodowska-Curie grant agreement under Contract No. 894790; German Research Foundation DFG under Contracts Nos. 443159800, 455635585, Collaborative Research Center CRC 1044, FOR5327, GRK 2149; Istituto Nazionale di Fisica Nucleare, Italy; Ministry of Development of Turkey under Contract No. DPT2006K-120470; National Research Foundation of Korea under Contract No. NRF-2022R1A2C1092335; National Science and Technology fund of Mongolia; National Science Research and Innovation Fund (NSRF) via the Program Management Unit for Human Resources \& Institutional Development, Research and Innovation of Thailand under Contract No. B16F640076; Polish National Science Centre under Contract No. 2019/35/O/ST2/02907; The Swedish Research Council; U. S. Department of Energy under Contract No. DE-FG02-05ER41374

\textbf{Other Fund Information}

To be inserted with an additional sentence into papers that are relevant to the topic of special funding for specific topics. Authors can suggest which to Li Weiguo and/or the physics coordinator.
        Example added sentence: This paper is also supported by the NSFC under Contract Nos. 10805053, 10979059, ....National Natural Science Foundation of China (NSFC), 10805053, PWANational Natural Science Foundation of China (NSFC), 10979059, Lund弦碎裂强子化模型及其通用强子产生器研究National Natural Science Foundation of China (NSFC), 10775075, National Natural Science Foundation of China (NSFC), 10979012, baryonsNational Natural Science Foundation of China (NSFC), 10979038, charmoniumNational Natural Science Foundation of China (NSFC), 10905034, psi(2S)->B BbarNational Natural Science Foundation of China (NSFC), 10975093, D 介子National Natural Science Foundation of China (NSFC), 10979033, psi(2S)->VPNational Natural Science Foundation of China (NSFC), 10979058, hcNational Natural Science Foundation of China (NSFC), 10975143, charmonium rare decays
%% ends here %%

